Deontic Meta-Rules

The use of meta-rules in logic, i.e., rules whose content includes other rules, has recently gained attention in the setting of non-monotonic reasoning: a first logical formalisation and efficient algorithms to compute the (meta)-extensions of such theories were proposed in Olivieri et al (2021) This work extends such a logical framework by considering the deontic aspect. The resulting logic will not just be able to model policies but also tackle well-known aspects that occur in numerous legal systems. The use of Defeasible Logic (DL) to model meta-rules in the application area we just alluded to has been investigated. Within this line of research, the study mentioned above was not focusing on the general computational properties of meta-rules. This study fills this gap with two major contributions. First, we introduce and formalise two variants of Defeasible Deontic Logic with Meta-Rules to represent (1) defeasible meta-theories with deontic modalities, and (2) two different types of conflicts among rules: Simple Conflict Defeasible Deontic Logic, and Cautious Conflict Defeasible Deontic Logic. Second, we advance efficient algorithms to compute the extensions for both variants.

==> Intro.tex <==


An extensive research has been devoted in the AI community for developing rule-based systems in the normative domain. It is widely acknowledged that norms have, basically, a conditional structure like
\[
\text{if } a_1,\dots ,a_n \text{ then } b
\]
where $a_1,\dots ,a_n$ are the applicability conditions of the norm, and $b$ denotes the legal effect which ought to follow when those applicability conditions hold. This, very general, view highlights an immediate link between the concepts of norm and rule.

This paper develops, in the context of normative reasoning, a rule-based logical framework providing an efficient computation of meta-rules, i.e., rules having rules as their elements. We shall proceed with the simple idea that a rule is nothing but a (binary) relationship between a set of conditions, and a conclusion. The meaning of such a relationship is to determine under which conditions a conclusion can be derived. Meta-rules thus generalise such an idea by establishing that, in addition to standard conclusions, rules themselves can be the ``conclusion'', and elements of the set of conditions. In other terms, new rules can be generated from other rules, along with conditions that are not rules per se.

While the meaning of meta-rules was formally investigated in  mathematical logic (see Section~\ref{sec:RelatedWork} for a discussion), the philosophical issue of admitting meta-rules in the logical language was critically discussed for a long time in conditional logics \cite{nute:1980}. At the end of the `60, such logics have been studied to give formal account to linguistic structures such as indicative conditionals and subjunctive conditionals to express counterfactuals. Later on, conditional logics  have been also used to deal with a non-monotonic reasoning \cite{Delgrande:87,Farinas:94}. While some,  like \cite{adams:1975}, rejected nested rules when a probabilistic treatment of conditionals is considered, others admitted this possibility even though it was argued that the intuitive meaning of such formulas is not clear \cite{Lewis:1973,nute:1980,Delgrande:87}. Some made some proposals about the meaningful use of nested conditionals \cite{Boutilier:92}.

If we move to the normative domain, an interesting discussion can be developed, since meta-rules (or rules with nested rules) occur frequently in normative reasoning and policies for security systems. 
Very often, when a set of policies is represented by a set of rules, we have to consider the policy that contains conditions (rules) about \emph{itself} (and also about other sets of rules/policies). Consider the example in \cite{ruleml05insu}, where a company has a security policy specifying that: (i) a piece of information is deemed confidential when its disclosure would harm the interests of the company, and that (ii) confidential information must be protected (and hence cannot be disclosed). Such a policy can be naturally represented by the meta-rule
\[
 \big(\mathit{Disclose}(x) \rightarrow \mathit{HarmInterests}\big) \rightarrow \mathit{Confidential}(x).
\]
%
Now, in this policy, the condition about harming the interests should be represented by an hypothetical expression: an `$\textsc{If}\, (\dots)\, \textsc{Then}\, (\dots)$' rule would appear to be the most natural way to represent such a construct. Furthermore, the hypothesis is part of the conditions to define when a piece of information is confidential (in this case, is the condition itself). Unfortunately, we cannot use classical material implication ($\supset$), given its well-known paradoxes. Consequently, if we model the policy as
\[
  (\mathit{Disclose}(x) \supset \mathit{HarmInterests}) \rightarrow \mathit{Confidential}(x),
\]
%
given the equivalence between $\mathit{Disclose}(x) \supset \mathit{HarmInterests}$ and $\neg\mathit{Disclose}(x) \vee \mathit{HarmInterests}$, we have the counter-intuitive scenarios where (1) if $x$ is not disclosed then $x$ is confidential (information that is not confidential, no matter if disclosed or not, it does not need to be protected), and (2) if, for any reason, company interests are harmed, then $x$ is confidential, for any piece of information. The policy can neither be defined as 
\[
  \big(\mathit{Disclose}(x) \wedge \mathit{HarmInterests}\big) \rightarrow \mathit{Confidential}(x)
\]
%
given that a disclosed information (with the consequent harm of interests) can no longer be considered confidential. 

Another situation where meta-rules are useful occurs when the inclusion of a rule in a set of rules depends upon whether other rules are already in the system. For instance, we can have
\[
 r_1 \rightarrow r_2,
\]
%
indicating that the existence of rule $r_2$ in the system depends on the  existence in the system of rule $r_1$. For instance,
this could be the case of an \emph{implementing decree} whose mere existence depends upon the existence of the 
law whose prescriptions are indeed implemented.
 
Typically, such dependencies among rules are stored externally, but if we model them directly into the system by using meta-rules, then we can include (or remove) $r_2$ automatically, based on the other rules it depends upon (and thus automatising the system's maintenance functionalities). In addition, this feature is beneficial to system integration, as it supports context-dependent rules. 
The definition of context-dependent policies is valuable in many situations; for instance, the defence forces of a country can have different rules of engagement, depending on the environment in which they are situated. One might think that a simple (and somehow naive) way to achieve this would be to partition the rules into independent rule sets, one for each context, and then to use simpler rules (without nested rules). However, as discussed, there could be dependencies among the rules, and the environments themselves can be defined in terms of rules. Accordingly, a clear partition of the simple rules might not be feasible. 


Another area of legal reasoning, where meta-rules proved to be essential in representing the legal processes at hand, is related to the of field of norm change. As we argued, many legislative instruments contain provisions (norms) about who has the power to create, modify, revoke, or abrogate other norms. If norms can be represented as rules \cite{Sartor05}, and there are norms `speaking about other norms', then it would be natural to have rules whose content consists of other rules. 

Different variants of Defeasible Logic have been proposed \cite{igpl10normchange,Cristani201739} to incorporate meta-rules in order to describe the logical behaviour of norm changes. An important aspect of norm changes is that some legal systems can specify that certain norms cannot exist (or cannot be in force) in that particular legal system. For instance, in the Italian Constitution, Article 27 prescribes that there cannot be norms in the Italian legal system prescribing Capital Punishment. This means that a meta-norm can speak about the positive existence of a rule, as well as preventing a rule to be generated in the system itself after the enforcement of the meta-norm.  

Finally, meta-rules have been proposed to model private international law, which is the body of rules and principles governing the choice of law to be applied, when there are conflicts in the domestic law of different countries related to private legal facts and transactions \cite{stone}. Works such as \cite{DungS11,MalerbaRG16,Rotolo:2021} argued that we need a reasoning mechanism that allows us to conclude that, if something holds in some legal system, then some norm holds in this or another legal system, or that allows us to import, in a given system, any piece of information holding in another system. Meta-rules are thus relevant in order to model such
an interaction.

In this paper, we extensively study a new computational framework (based on a variant of Defeasible Deontic Logic) that models rules and meta-rules for the normative domain. We shall distinguish between the content of a rule (which is a binary relationship between a set of premises and a conclusion, both represented as propositions in an underlying, given language), and the name, or identifier, of the rule itself. In this set up, a rule can be understood as a function associating a label to the content of the rule. Similarly, a meta-rule is a function that associates the name, or label, to the content, but in this case the elements of the binary relationship corresponding to the content of the meta-rule can contain other rules. 

In addition,  we shall admit \emph{negation of rules}. If we are able to conclude that a (positive) rule holds, then it means that we can insert the rule (the content of the rule, with a specific name) in the system, and we can use the resulting rule to derive new conclusions. For a negated rule, the meaning is that it is not possible to obtain a rule with that specific content (this can be either formally prescribed for the whole rule, or in a way that results irrespective of the name). 
The analysis of the specific aspects involving the possible (diverse) ways of evaluating and using the negation of rules
is dealt with in this paper with care, for this is one important issue in the development of reasoning methods
for these logical systems.


The paper is structured as follows. 
Section \ref{sec:basic_ideas} provides a discussion that frames meta-rules in legal reasoning.
Section \ref{sec:Method} is devoted to introduce the methodological issues
of the investigation, and to discuss the basic structure of Defeasible Deontic Logic, including proof theory associated
to it. In Section \ref{sec:Logic} we formally provide the meta-logical framework that is the subject of the investigation 
documented in this paper. The theoretical framework is then considered from a computational problem in Section \ref{sec:Algo},
where algorithms to compute meta-extensions and extensions are provided, and analysed from a correctness/completeness and
complexity viewpoints. Section \ref{sec:RelatedWork} reviews current relevant literature, and Section \ref{sec:Conc}
takes some conclusions and discusses how this research can be taken further.




\section{Synopsis}\label{sec:synopsis}
In devising a new computational logical system for meta-rules in deontic reasoning we adopt the following roadmap and take the following steps:
\begin{itemize}
  \item we offer a conceptual analysis of meta-reasoning in the normative domain;
  \item we present the new logic;
  \item we investigate the computational properties of the logic.
\end{itemize}  

First of all, we need to set up a conceptual framework (Section \ref{sec:conceptual_framework}), where some basic philosophical problems are discussed and which is the basis of our formal choices. For the sake of illustration, just consider the complexities behind the definition of norm change mechanisms in domains such as the law or the interplay of norm dynamics and deontic concepts  such as permissions and permissive norms. 

Once this is done, we need to introduce the formalism that we use for modelling deontic and normative reasoning and to which meta-rules are added. Such a formalism must move from the above-mentioned conceptual analysis and be as richest as possible. This is done in Sections \ref{sec:Method} and \ref{sec:Logic}: the logic is an extension of a Defeasible Deontic Logic where we can  (a) represent the distinction between rules and meta-rules, (b) model the distinction between constitutive and deontic rules, (c) handle complex reasoning patterns related to contrary-to-duty and compensatory obligations, and various types of deontic statements.

Finally, we expect the logic be as well computationally efficient. Thus, we have to study the properties of the resulting system---and in particular, its computational behaviour---a study which is offered in Section  \ref{sec:Algo},
where algorithms to compute meta-extensions and extensions are provided, and analysed from a correctness/completeness and complexity viewpoints.  

The paper is thus structured as follows. 
Section \ref{sec:conceptual_framework} provides a discussion that frames meta-rules in legal reasoning.
Section \ref{sec:Method} is devoted to introduce the methodological issues
of the investigation, and to discuss the basic structure of Defeasible Deontic Logic, including proof theory associated
to it. In Section \ref{sec:Logic} we formally provide the meta-logical framework that is the subject of the investigation 
documented in this paper. The theoretical framework is then considered from a computational problem in Section \ref{sec:Algo},
where algorithms to compute meta-extensions and extensions are provided, and analysed from a correctness/completeness and
complexity viewpoints. Section \ref{sec:RelatedWork} reviews current relevant literature, and Section \ref{sec:Conc}
takes some conclusions and discusses how this research can be taken further.


\section{The Conceptual Framework}\label{sec:conceptual_framework}
%
\cite{igpl10normchange} argued that meta-rules describe the dynamics of any normative institution (such as a legal system) on which norms are formalised and can be used to establish conditions for the creation and modification of other rules or norms, while proper rules correspond to norms in a normative system. In particular, it was pointed out that meta-rules can be represented in the language of Defeasible Logic as follows 
%
\begin{gather*}
mr_1\colon\xseq{a}{n}\To (r_1:\xseq{b}{m}\To c)
\end{gather*}
%
precisely to grasp norm change mechanisms in the law. For instance, if the rule `$r_1:\xseq{b}{m}\To c$' does not exist in the theory at hand, then the successful application of $mr_1$ leads to derive such a rule, which amounts to enact $r_1$ as a new norm in the legal system. Similarly, if $r_1$ already exists but has the form `$r_1\colon b_1\To c$', then the successful application of $mr_1$ corresponds to modifying $r_1$ from `$r_1\colon b_1\To c$' to `$r_1\colon\xseq{b}{m}\To c$'.

In addition,  with meta-rules we can admit the \emph{negation of rules}. If we are able to conclude that a (positive) rule holds, then it means that we can insert the rule (the content of the rule, with a specific name) in the system, and we can use the resulting rule to derive new conclusions. For a negated rule, the meaning is that it is not possible to obtain a rule with that specific content (this can be either formally prescribed for the whole rule, or in a way that results irrespective of the name). 


In this paper, we go further and discuss the conceptual meaning of modalising rules via meta-rules, i.e., what we mean when we establish the obligatoriness of the enactment of a certain rule. Put in this way, making a rule obligatory in fact amounts to firing a meta-rules like the following:
%
\begin{gather*}
mr_2\colon \xseq{a}{n}\To_{\Obl} (r_2\colon\xseq{b}{m}\To_{\Obl} c).
\end{gather*}
%
Rule $r_2$ is a standard deontic rule as described in previous works \cite{GovernatoriOSRC16,GovernatoriORS13,GovernatoriR08}: if $\xseq{a}{n}$ are the case, then rule $r_2$ allows us to derive that $c$ is obligatory. If a similar intuition is extended to meta-rules, then $mr_2$ asserts that enacting rule `$r_2\colon\xseq{b}{m}\To_{\Obl} c$' is obligatory.

We should now ask: For whom `$r_2\colon\xseq{b}{m}\To_{\Obl} c$' is obligatory? There is no unique answer, since the question has different meanings depending on which normative domain is considered. If we work, again, in the legal domain, we can imagine that a legislative authority imposes the obligation to enact a certain norm over another authority, lower in the legislative hierarchy but competent in enacting such a norm. Concrete examples occur in the law, when, for instance, European authorities impose to  member states the implementation of European directives, or when Constitutional courts require national parliaments to amend, or to integrate, the legislative corpus. 

We should note that  structures like $mr_2$ do not lead to a meaningless iteration of deontic modalities, an issue that was explored in early deontic literature such as in \cite{Barcan:1966,Goble:1966}. Indeed, while it looks meaningless to have an expression like $\Obl \Obl c$ standing for ``It is obligatory that it is obligatory that everyone keeps their promises'', an expression like ``Parking on highways ought to be forbidden'' makes sense \cite{Barcan:1966}. This second example  suggests that a norm forbidding to park in highways is obligatory, thus assuming a conceptual distinction between norms, on one side, and obligations (and permissions), on the other side \cite{alchourron71normative}.  This general approach, hence, clearly distinguishes norms from obligations:  obligations are the effects (i.e., the conclusions) of the application of prescriptive norms. Under this reading, the application of rule $r_2$ leads the obligation $\Obl c$, while the application of meta-rule $mr_2$ leads to state that norm $r_2$ ought to be the case.

What about the permission? The elusive character of permission affects also the case of permissive meta-rules. Consider this meta-rule:
%
\begin{gather*}
mr_3\colon \xseq{a}{n}\To_{\Perm} (r_2\colon\xseq{b}{m}\To_{\Obl} c).
\end{gather*}
%
Does the well-known distinction between \emph{weak}
and \emph{strong} permission \cite{vonwright:1963} apply to this case as well? In the standard scenario, the former type of permission corresponds to saying that something is allowed by a code precisely when it is not prohibited by that code. This idea is preserved when meta-rules are considered. Indeed, one may simply argue that, if the legal system \emph{does not} support the derivation of 
\begin{gather*}
\Obl\neg(r_2\colon\xseq{b}{m}\To_{\Obl} c)\\
\Obl(r_3\colon\xseq{b}{m}\To_{\Obl} \neg c)
\end{gather*}
%
then one may also conclude that the following holds:
\begin{gather*}
\Perm (r_2\colon\xseq{b}{m}\To_{\Obl} c).
\end{gather*}
%
For similar reasons, since weak permission is the dual of obligation---i.e., $\Obl A =_{\mathit{def}} \neg \Obl \neg A$---imposing consistency means $\Obl A \to \Perm A$,  and so it looks reasonable that from $\Obl(r_2:\xseq{b}{m}\To_{\Obl} c)$ we can 
obtain $\Perm (r_2:\xseq{b}{m}\To_{\Obl} c)$.

As is well-known, the concept of strong permission is more complicated, as it
amounts to saying that some $a$ is permitted by a code iff such a
code explicitly states that $a$ is permitted. Various sub-types of permissions can be thus identified, such as the following ones \cite{makinson-torre:2003,boella-torre-icail:2003,stolpe-jal:2010,GovernatoriORS13}:
%
\begin{description}
\item[Static permission:] $X$ is a static permission wrt a normative system when
$X$ is derived from a strong permission, i.e., from an explicit permissive norm;
\item[Dynamic permission:] $X$ is a dynamic permission wrt a normative system 
 when it guides the legislator by describing the limits on what may be prohibited typically without violating static permissions in the system;
 \item[Exemption:] $X$ is an exemption wrt a normative system
  when it is an exception of a prohibition contained in the system.
\end{description}

It seems reasonable that all these types may be extended to the case of meta-rules. The first case simply amounts to when a rule is explicitly permitted in the theory or it is derived from a permissive meta-rule (such as $mr_3$). The third case is when, for instance, we have in the system two rules such as 
\begin{gather*}
\Perm (r_2:\xseq{b}{m}\To_{\Obl} c)\\
\Obl (r_3:\xseq{b}{m}\To_{\Obl} \neg c)
\end{gather*}
and we know that $r_2$ is stronger than $r_3$ or, at a meta-rule level, we have
%
\begin{gather*}
mr_3: \xseq{a}{n}\To_{\Perm} (r_2:\xseq{b}{m}\To_{\Obl} c) \\
mr_4: \xseq{a}{n}\To_{\Obl} (r_3:\xseq{b}{m}\To_{\Obl} \neg c) 
\end{gather*}
%
and, similarly, $mr_3$ is stronger than $mr_4$. The idea of dynamic permission consists in preventing the theory from deriving any incompatible deontic rule, for example, by setting that the meta-rule $mr_3$ is stronger than any other meta-rule supporting any conflicting rule. 

The discussion above shows how it is crucial to establish some logical properties of permitted rules and 
to determine when modalised rules are in conflict. 

Accordingly, desirable basic properties are the following ones:
%
\begin{gather}
\Perm (\xseq{a}{n}\To_{\Obl} b) \vdash \neg\Obl(\xseq{a}{n}\To_{\Obl} \neg b) \label{eq:reviewer1}\\
\Perm (\xseq{a}{n}\To_{\Box} b) \vdash \neg\Obl \neg (\xseq{a}{n}\To_{\Box} b) \label{eq:reviewer2}
\end{gather} 

\sloppy (\ref{eq:reviewer2}) is trivially desirable because $\Perm \phi$ should imply $\neg \Obl \neg \phi$ even when $\phi$ is a rule. Instead, if the rule in the scope of the permission is a permissive norm---i.e., $\xseq{a}{n}\To_{\Perm} b$---the  principle (\ref{eq:reviewer1}) does not hold\footnote{Many thanks to a reviewer for commenting on this point.}. Suppose that the normative system (for example, on the basis of constitutional values) permits the enactment of a norm which allows for the temporary limitation of liberties due to public health reasons. If so, it would not be contradictory to have that the normative system prescribes that the lack of limitation is also permitted. The following rules are in fact not necessarily incompatible:
%
\begin{gather*}
\mathit{public\_health}\To_{\Perm} \mathit{limit\_liberties}\\
\mathit{public\_health}\To_{\Perm} \neg \mathit{limit\_liberties}
\end{gather*} 
%
which, essentially, amount to saying that $\Perm \mathit{limit\_liberties}$ and $\Perm \neg \mathit{limit\_liberties}$ are deontically compatible.


Other properties depend on at to what extent we assume that legislator was rational in a subtler way. For instance, the following one
%
\begin{gather}
\Perm (\xseq{a}{n}\To_{\Obl} b) \vdash \neg\Perm (\xseq{a}{n}\To_{\Obl} \neg b) \label{eq:DPermRuleInternal}
\end{gather}
can be rational, since it does not make much sense for a rational legislator to permit that two deontically incompatible rules are the case. 

Let us discuss the case of (\ref{eq:DPermRuleInternal}). If we accept it, one may similarly argue that we should also adopt the following (where $b$ is a literal):
%
\begin{gather}
\Perm  b \vdash \neg\Perm \neg b \label{eq:D_Perm}
\end{gather}
%
which, however, cannot be accepted. Why? As we know, the deontic facultativeness of a certain $b$ precisely amounts to stating $\Perm  b \wedge \Perm \neg b$, so  (\ref{eq:D_Perm}) would make facultativeness inconsistent.

What about facultative norms? We may have two cases like the following ones:
\begin{gather}
\Perm (\xseq{a}{n}\To_{\Obl} b) \qquad \Perm \neg (\xseq{a}{n}\To_{\Obl}  b) \label{eq:FacultativeRule1} \\
\Perm (\xseq{a}{n}\To_{\Obl} b) \qquad \Perm (\xseq{a}{n}\To_{\Obl}  \neg b). \label{eq:FacultativeRule2}%\\
\end{gather}
Clearly, (\ref{eq:FacultativeRule1}) and (\ref{eq:FacultativeRule2}) are deontically different. While the former states that 
% the enactment of
$\xseq{a}{n}\To_{\Obl} b$ is facultative, the latter says that two deontically incompatible and different rules are permitted. What is facultative according to (\ref{eq:FacultativeRule2})? Certainly we cannot say that  $\Obl b$ is facultative, since we would need to permit two rules, one supporting $\Obl b$---which is the case: $\xseq{a}{n}\To_{\Obl} b$---and one supporting $\neg \Obl b$---which we do not have. (\ref{eq:FacultativeRule2}) licenses that both $\Obl b$ and $\Obl \neg b$ are permitted given $\xseq{a}{n}$. Is it factually possible? Yes, it is. Is it deontically admissible? Perhaps, it is. Is it always deontically rational? We have sometimes arguments to answer No. 

Consider the idea of static permission. Assume we would like to avoid having two deontically incompatible rules in the system. Then, it would not be reasonable to explicitly permit that both rules are the case. Precisely as in skeptical defeasible reasoning, if we have arguments for deriving $b$ and $\neg b$ we refrain from concluding anything on the assumption that $b$ and $\neg b$ are in contradiction, we could reason similarly when two conflicting deontic rules like $\xseq{a}{n}\To_{\Obl} b$ and $\xseq{a}{n}\To_{\Obl} \neg b$ are considered.  

Consider instead the idea of dynamic permission: the aim here is limiting the legislator in dynamically adding prohibitions. If so, 
\begin{gather*}
\Perm (\xseq{a}{n}\To_{\Obl} b) \text{ prevents the derivation of }\xseq{a}{n}\To_{\Obl} \neg b\\
\Perm (\xseq{a}{n}\To_{\Obl} \neg b) \text{ prevents the derivation of }\xseq{a}{n}\To_{\Obl} b.
\end{gather*}
If we have it, it means that we want the system to be deontically indifferent with respect to $b$ whenever $\xseq{a}{n}$ are the case. But suppose that we also have two norms like the following:
%
\begin{gather*}
\xseq{a}{n}\To_{\Obl} c \\
\Obl c \To_{\Obl} b
\end{gather*}
%
Can we still say that the system is deontically indifferent with respect to $b$ given $\xseq{a}{n}$?

Accordingly, under the reading above, one may prudentially establish that the following meta-rules are in conflict:
%
\begin{gather}
mr_3\colon \xseq{a}{n}\To_{\Perm} (r_2\colon\xseq{b}{m}\To_{\Obl} c) \label{eq:1}\\
mr_5\colon \xseq{a}{n}\To_{\Perm} (r_3\colon\xseq{b}{m}\To_{\Obl} \neg c) \label{eq:-1} 
\end{gather}

%
Clearly, we assume in the above discussion that $\Perm$ is not the dual of $\Obl$, but rather as another $\Box$-operator. A logic for meta-rules assuming that \ref{eq:1} and \ref{eq:-1} \emph{are in conflict} is named \textbf{prudential}.

On the contrary, if we believe that the permission, as applied to rules, behaves exactly as when literals are modalised, then $mr_3$ and $mr_5$ are not in conflict, and this holds precisely because
%
\begin{gather}
r_4\colon \xseq{a}{n}\To_{\Perm} b\\
r_5\colon \xseq{a}{n}\To_{\Perm} \neg b 
\end{gather}
%
are likewise compatible in virtue of the intuition that $\Perm b$ and $\Perm \neg b$ are consistent. A logic for meta-rules assuming that \ref{eq:1} and \ref{eq:-1} \emph{are not in conflict} is named \textbf{simple}.

Let us finally comment on the application of the $\otimes$ operator \cite{GovernatoriORS13} to rules. In the standard reading of this operator, a rule like
$\xseq{a}{n}\To_{\Obl} b\otimes c$ means that if $\xseq{a}{n}$ are the case, then $b$ is
obligatory, but if the obligation $b$ is not fulfilled, then the obligation
$c$ is activated and becomes in force until it is satisfied, or violated. Since we argued that a legislator $L_1$ can impose to another legislator $L_2$ to enact a norm $r_1$, we can imagine a scenario where $L_2$ violates $\Obl r$, but we can also imagine that $L_1$ has considered a sanction as the result of such a violation, or rather that another normative solution is advanced by $L_2$. Accordingly, expressions such as
%
\begin{gather}
mr_6\colon \xseq{a}{n}\To_{\Obl} (r_2:\xseq{b}{m}\To_{\Obl} c)\otimes (r_6\colon \xseq{b}{m} \To_{\Obl} d)
\end{gather}
%
are admissible. 
%
The $\otimes$ operator can be also seen as a preference operator, where the first element is the most preferred and the last is the least of the acceptable options \cite{GovernatoriORS13,GovernatoriOSRC16}. According to this reading, meta-rule $mr_6$ establishes that the underlying normative systems should introduce rule $r_2$ (if such a rule is not already in the system). Alternatively, a less preferable but still acceptable outcome is to impose $r_6$. Generally, in real-life normative systems, the idea is to use this kind of structure to prescribe more and more stringent norms/policies.  


  



